Categorical Foundations of Gradient-Based Learning

We propose a categorical semantics of gradient-based machine learning algorithms in terms of lenses, parametrised maps, and reverse derivative categories. This foundation provides a powerful explanatory and unifying framework: it encompasses a variety of gradient descent algorithms such as ADAM, AdaGrad, and Nesterov momentum, as well as a variety of loss functions such as as MSE and Softmax cross-entropy, shedding new light on their similarities and differences. Our approach to gradient-based learning has examples generalising beyond the familiar continuous domains (modelled in categories of smooth maps) and can be realized in the discrete setting of boolean circuits. Finally, we demonstrate the practical significance of our framework with an implementation in Python.

==> case-studies.tex <==

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

Do we still have a section like this?  One reviewer for ACT did comment it was very helpful...

==> composing-learners.tex <==

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

Not needed anymore - or do we discuss just composing networks and applying R to them?  

==> introduction.tex <==

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

==> para.tex <==
We proceed to recall the definition of the double category $\Dbl{\Ca}$ from
\cite{DelayedTrace} \footnote{Interestingly, we note that $\Dbl{\Ca}$ has the
  same data as the \textit{bicategory of processes} defined in \cite[Sec.
  2.1]{BicatOfProcesses}.}, and note that their restriction to a strict
Cartesian one is needlessly concrete: the construction works with any strict symmetric monoidal category.

\begin{definition}[compare \cite{DelayedTrace}, Def. 1]
Let  $\Ca$ be a strict symmetric monoidal category. Then we can form a double
category $\Dbl{\Ca}$ with a unique 0-cell, and whose vertical and horizontal
1-cells are given by objects of $\Ca$. A 2-cell with a source horizontal 1-cell
$P$, targer horizontal 1-cell $Q$, source vertical 1-cell $X$ and target
vertical 1-cell $Y$ \footnote{Following the convention in \cite{DelayedTrace}, the horizontal 1-cells are on top and bottom of a 2-cell square, the vertical ones are on the
left and the right.}is a morphism $f : P \otimes X \to Q \otimes Y$ in $\Ca$.
The compositions are defined as in \cite[Def. 1]{DelayedTrace}.
\end{definition}

The double-categorical variant allows us to use a two-dimensional graphical
language described in Myers' \cite{StringDiagramsDoubleCat}. The full-blown
graphical language of Myers' is not needed: since our double category has a
unique 0-cell, we do not need to use any colors. 

We are now ready to show that $\Para{\Ca}$ is double category too. 

\begin{proposition}
The bicategory $\Para{\Ca}$ is sub-double category of $\Dbl{\Ca}$, with the same
vertical and horizontal 1-cells, but whose 2-cells all have the target horizontal 1-cell the monoidal unit $I$ of $\Ca$.
\end{proposition}

This allows us to use Myers' two dimensional tiling language for $\Para{\Ca}$.
We can also think of $\Para{\Ca}$ as a bicategory, and correspondingly interpret
what the 0-cells, 1-cells and 2-cells mean: 0-cells $X$ and $Y$ become left and
right edges of a tile, a 1-cell (a choice of a parameter $P$ and a map $f : P
\otimes X \to Y$) becomes the tile itself (whose top edge is $P$ and bottom $I$)
and a 2-cell $\alpha : (P, f) \Rightarrow (Q, g)$ becomes a tile on top of $f$,
whose top edge is $Q$, bottom $P$, and left and right edges are $I$.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


